The Geometry of Distributed Representations for Better Alignment, Attenuated Bias, and Improved Interpretability

High-dimensional representations for words, text, images, knowledge graphs and other structured data are commonly used in different paradigms of machine learning and data mining. These representations have different degrees of interpretability, with efficient distributed representations coming at the cost of the loss of feature to dimension mapping. This implies that there is obfuscation in the way concepts are captured in these embedding spaces. Its effects are seen in many representations and tasks, one particularly problematic one being in language representations where the societal biases, learned from underlying data, are captured and occluded in unknown dimensions and subspaces. As a result, invalid associations (such as different races and their association with a polar notion of good versus bad) are made and propagated by the representations, leading to unfair outcomes in different tasks where they are used. This work addresses some of these problems pertaining to the transparency and interpretability of such representations. A primary focus is the detection, quantification, and mitigation of socially biased associations in language representation.

==> abstract.tex <==


High-dimensional representations for words, text, images, knowledge graphs and other structured data are commonly used in different paradigms of machine learning and data mining. These representations have different degrees of interpretability, with efficient distributed representations coming at the cost of the loss of feature to dimension mapping. This implies that there is obfuscation in the way concepts are captured in these embedding spaces. Its effects are seen in many representations and tasks, one particularly problematic one being in language representations where the societal biases, learned from underlying data, are captured and occluded in unknown dimensions and subspaces. As a result, invalid associations (such as different races and their association with a polar notion of good versus bad) are made and propagated by the representations, leading to unfair outcomes in different tasks where they are used.

This dissertation addresses some of these problems pertaining to the transparency and interpretability of such representations. A primary focus is the detection, quantification, and mitigation of socially biased associations in language representation.
First, using the underlying geometrical structure of the high-dimensional space occupied by the representations, we build an understanding of the relative orientation between point sets. Next, we capture and isolate different feature subspaces or concept subspaces (such as gender or occupations in language representations) within the embedding space. Following this, we develop methods to decouple specific subspaces so as to better prepare the representations for specific downstream tasks. We also build a comprehensive range of probes to understand and highlight the different implicit associations learnt by the representations from underlying data, as an effort to distinguish between meaningful and invalid associations learnt and amplified by the embeddings. This is especially impactful as these representations drive much of the tasks and real world applications based on Natural Language Processing.
 Finally, we extend and apply these methods to different distributed representations and demonstrate the applications of increased interpretability. 


==> acknowledge.tex <==

I am extremely thankful for the consistent advice, guidance, and support of my advisor, Jeff M Phillips, without which this dissertation would not have been possible. I feel very fortunate to have had a mentor who was not just extremely erudite but also incredibly kind. While his timely guidance and infallible intuition always helped me gain direction in my projects, his immense compassion and tireless patience helped make a better researcher out of me. I learnt from him not just how to approach and answer a research question but also how to astutely ask the right questions.

I am also very grateful to my committee for their invaluable input. I feel very lucky to have had the opportunity to work with Vivek Srikumar and learn so much from him, most importantly, the right way to think about language tools. I am thankful for the holistic understanding of the pursuit of responsible AI that Suresh Venkatasubramanian introduced me to in so many ways. I am especially grateful to both of them for the time they took to provide me with acute critique of my work which helped nudge me toward the right questions to answer. I was also lucky to have worked with Yan Zheng at Visa Research, where she was not just a wonderful mentor with great insights but a kind friend. I am extremely grateful for the time and input Kai-Wei Chang provided me with whenever I reached out to him and for the opportunities for future work that he has helped open up for me.

I am also grateful for the many enlightening interactions with Tao Li over the course of our collaboration. Working with him has been an extremely rewarding process. I would further like to thank all the other wonderful people I have had the chance to collaborate with and learn from: Wei Zhang and Michael Yeh at Visa Research, Haijing Wang, Yi Zhang, and Mehul Parsana at Microsoft and Bei Wang and Archit Rathore at the University of Utah.
 

Along this journey, I was lucky to have had so many wonderful friends by my side. I thank Sierra Allred, Sumanth Gudaparthi, and Greeshma Mahadeva Prasad for being my home in this strange new city. I am also indebted to Michael Matheny, Siddharth Ranade, Mohsen Abbasi, and Anirban Nag for the many lively discussions we had about work, math, research and life which made our lab such a welcoming place to come to every day. 

I thank Shantanu Thakar for being there through all my endless rants and fears, for his undying support, for never letting me lose hope through rejections and doubts and for making me aim higher than I trusted myself to. 
 
Finally, I cannot thank my family enough for their constant encouragement. My parents, Shibaprasad and Snigdha Deb for their absolute faith and unwavering pride in me and all I do and Shreya and Budhaditya Dev for being my biggest, personal cheerleaders. The support of my family has always given me the courage to pursue all my dreams.


==> notation.tex <==
%%% -*-LaTeX-*-
%%%
%%% This is notation.tex.
%%%
%%% This file is included in a thesis with a front-matter command
%%%
%%%     \optionalfront {Notation and Symbols} {\input{notation}}
%%%
%%% The heading for this material is provided by the first argument
%%% so none needs to be supplied here.

\begin{tabular}{ll}
    \hline
    $v$      & vector \\
    \textsf{word}       & word or token in data\\
    SVD(A)    & singular value decomposition of matrix A\\
    $\|v\|$    & norm of vector $v$\\
    
    
    \hline
\end{tabular}

